Circuit-Diff: Factual Edit-based Intervention Method for Localizing Knowledge in Attribution Graphs

Mechanistic interpretability defines features as the fundamental units of a neural network and circuits as the weighted subgraphs that carry out its computation. Because individual neurons are polysemantic, Cross-Layer Transcoders (CLTs) were introduced as a way to approximate a model's circuits by generating an attribution graph. The nodes of that graph, however, are unlabeled features: reading a graph means pruning it and then working out by hand what each surviving node means. To make CLTs easier to use for circuit discovery, we introduce Circuit-Diff, which intervenes on the model itself with a low-rank factual edit and takes the features whose role in the attribution graph changes under that edit as related to the edited knowledge. On the edits we examine, the flagged nodes are not only detectors of the object token: read off the CLT's released feature dashboards, they include features for the history, geography and associations surrounding the old and new objects. We formalize the method, measure how reliable a frozen CLT remains after a factual edit, test the selected nodes causally by patching them on up to 24 CounterFact edits, give a case study, and release an open-source implementation built on the circuit-tracer package, together with two further tools (multi-prompt aggregation and rule-based supernode labeling).

==> notation.tex <==
% =====================================================================
% notation.tex — Circuit-Diff paper notation macros
% Source of truth: NOTATION.md (ledger, resolved 2026-08-12).
% Usage: \input{notation} after the package block. All macros are math-mode
% unless noted. Rename a concept here, and the whole paper follows.
% =====================================================================

\RequirePackage{amsmath}   % \text, align, \operatorname — score equations need these

% ---- §1 Core objects -------------------------------------------------
\newcommand{\Mbase}{M_0}                       % base (unedited) model
\newcommand{\Medit}{M_e}                       % edited model
\newcommand{\Tbase}{T_0}                       % base transcoder (frozen lens when read on M_e)
\newcommand{\Tft}{T_f}                         % fine-tuned (adapted) transcoder
\newcommand{\graphof}[2]{G(#1,\,#2)}           % attribution-graph constructor G(M, T)
\newcommand{\graphofx}[3]{G(#1,\,#2;\,#3)}     % with explicit prompt: G(M, T; x)
\newcommand{\prompt}{x}                        % the prompt
\newcommand{\objold}{o}                        % old (true) object
\newcommand{\objnew}{o^{*}}                    % new (counterfactual) object
\newcommand{\ptok}[2]{p_{#1}(#2 \mid \prompt)} % token probability, e.g. \ptok{\Medit}{\objnew}

% ---- §2 Lens-grid cells (bare capitals mean ONLY these) --------------
\newcommand{\cellA}{A}                         % G(M_0, T_0)
\newcommand{\cellB}{B}                         % G(M_e, T_0)  — frozen lens on edited model
\newcommand{\cellC}{C}                         % G(M_e, T_f)
\newcommand{\cellD}{D}                         % G(M_0, T_f)  — control corner (a.k.a. legacy F_b)

% ---- §3 Graph internals ---------------------------------------------
% NODE CONVENTION (2026-08-14): node n = (i, t) — feature i at token position t.
% All graph quantities are node-indexed: a_n, \edge{n}{n'}, I_n, scores \scoreI{a}{n}.
% Lowercase n = node ONLY; trial count is capital N (\ntrials).
\newcommand{\virt}[2]{v_{#1 \to #2}}           % virtual weight, feature-level & input-invariant: \virt{i}{j}
\newcommand{\edge}[2]{w_{#1 \to #2}}           % edge weight BETWEEN NODES, prompt-specific: \edge{n}{n'}
\newcommand{\edgedist}[1]{\pi_{#1}}            % edge-importance distribution \edgedist{n}
\newcommand{\dI}[1]{\Delta I_{#1}}             % influence difference \dI{n}
\newcommand{\appearedset}{\mathcal{N}^{+}}     % appeared nodes
\newcommand{\disappearedset}{\mathcal{N}^{-}}  % disappeared nodes
\newcommand{\featref}[2]{\mathrm{L}#1/\mathrm{f}#2} % canonical feature reference \featref{18}{7269}
\newcommand{\noderef}[3]{\mathrm{L}#1/\mathrm{f}#2@\mathrm{t}#3} % node reference \noderef{18}{7269}{5} -> L18/f7269@t5
\newcommand{\actfn}[1]{g\!\left(#1\right)}     % activation nonlinearity, e.g. \actfn{\mathbf{w}^\top h}; define g = JumpReLU at first use

% ---- §4 Interventions & experiment structure -------------------------
\newcommand{\dose}{\lambda}                    % signed intervention strength (ONLY meaning of lambda)
\newcommand{\doseopt}{\lambda^{*}}             % pre-registered per-feature optimum
\newcommand{\nfacts}{k}                        % facts per model (edit batch size)
\newcommand{\ntrials}{N}                       % trial count, CAPITAL (lowercase n = node)
\newcommand{\topq}[1]{top-#1\%}                % text-mode selection quantile, \topq{5}
\newcommand{\band}{\mathcal{B}}                % edit layer band, \band = [3,10]
\newcommand{\lrft}{\eta}                       % CLT fine-tuning learning rate
\newcommand{\epsR}{\varepsilon_R}              % recovery denominator guard
\newcommand{\epsact}[1]{\varepsilon_{#1}}      % activation guard \epsact{n} = \tauact a_i^max (feature-level max)
\newcommand{\tauact}{\tau_a}                   % activation-guard threshold (tau alone = Kendall)

% ---- §5 Heuristic scores & baselines ---------------------------------
\newcommand{\score}[1]{\phi^{(#1)}}            % \score{a} … \score{e}, strict: \score{c*}
\newcommand{\scoreI}[2]{\phi^{(#1)}_{#2}}      % with feature index: \scoreI{a}{i}
\newcommand{\scoreact}{\phi_{\mathrm{act}}}    % activation baseline ranking
\newcommand{\scoreinf}{\phi_{\mathrm{inf}}}    % influence baseline ranking
\newcommand{\actdelta}[1]{\delta_{#1}}         % normalized activation movement

% ---- §6 Recovery & collateral metrics --------------------------------
\newcommand{\Rnew}{R_{\mathrm{new}}}
\newcommand{\Rold}{R_{\mathrm{old}}}
\newcommand{\RnewAdj}{R^{\mathrm{adj}}_{\mathrm{new}}}
\newcommand{\RoldAdj}{R^{\mathrm{adj}}_{\mathrm{old}}}
\newcommand{\Rznew}{R^{z}_{\mathrm{new}}}
\newcommand{\Rzold}{R^{z}_{\mathrm{old}}}
\newcommand{\KLoff}{\mathrm{KL}_{\mathrm{off}}}
\newcommand{\ppatch}[1]{p_{\mathrm{patch}}(#1)} % M_0 + feature intervention at strength lambda

% ---- §7 Graph-quality & similarity ------------------------------------
\newcommand{\CErec}{\mathrm{CE}_{\mathrm{rec}}}
\newcommand{\featcos}[2]{\cos(#1,\,#2)}        % feature cosine, e.g. \featcos{\cellA}{\cellB}
% Replacement score / completeness score: WORDS ONLY in prose and figures.
% Never abbreviate replacement score as RS (RS = CounterFact consistency).

% ---- Terminology (text-mode) ------------------------------------------
\newcommand{\circuitdiff}{Circuit-Diff}        % the method name, one hyphenation everywhere
\newcommand{\frozenlens}{frozen lens}          % = \Tbase read on \Medit (i.e., cell B)
\newcommand{\adaptedlens}{adapted lens}        % = \Tft

